Poisson Flow Generative Models

We propose a new "Poisson flow" generative model (PFGM) that maps a uniform distribution on a high-dimensional hemisphere into any data distribution. We interpret the data points as electrical charges on the $z=0$ hyperplane in a space augmented with an additional dimension $z$, generating a high-dimensional electric field (the gradient of the solution to Poisson equation). We prove that if these charges flow upward along electric field lines, their initial distribution in the $z=0$ plane transforms into a distribution on the hemisphere of radius $r$ that becomes uniform in the $r \to\infty$ limit. To learn the bijective transformation, we estimate the normalized field in the augmented space. For sampling, we devise a backward ODE that is anchored by the physically meaningful additional dimension: the samples hit the unaugmented data manifold when the $z$ reaches zero. Experimentally, PFGM achieves current state-of-the-art performance among the normalizing flow models on CIFAR-10, with an Inception score of $9.68$ and a FID score of $2.35$. It also performs on par with the state-of-the-art SDE approaches while offering $10\times $ to $20 \times$ acceleration on image generation tasks. Additionally, PFGM appears more tolerant of estimation errors on a weaker network architecture and robust to the step size in the Euler method. The code is available at https://github.com/Newbeeer/poisson_flow .

==> dump.tex <==
\section{Physics Background}
A point charge $q_i$ placed at $x_i\in\mathbb{R}^n$ produces the electric field $E_i(y) = q_i(y-x_i)/||y-x_i||_2^{n}$. When $q_i<0$, the electric field starts from infinity and ends at the point charge, see Figure 1(a). More intuitively, if we release a positive test particle from a random point on the infinite ball, the test particle will follow the electric field and finally hit the point charge.  When multiple negative point charges are present, the electric field are simple additions of electric fields by single charges, i.e,
\begin{equation}
    E(y) = \sum_{i} E_i(y) = \sum_{i} q_i\frac{y-x_i}{||y-x_i||_2^n}
\end{equation}
We now ask: if we release a test particle whose initial position is drawn from the uniform distribution on the infinite sphere, and let the particle move along the electric field as $\dot{y}=E(y)$, where will the particle end up? The answer is: the particle will finally hit a point charge, and the probability to hit $q_i$ is $|q_i|/|Q|$ where $Q=\sum_i q_i$.


First, the particle will eventually be static rather than in motion because the potential $\phi$ ( which satisfies $E=-\nabla\phi$) decreases monotonically, so cyclic behavior is impossible. Secondly, we explain why the test particle will hit a point charge with probability one. What we mean by `hit a point $x$' is that the particle does not only arrive at the point $x$ but also is stable with respect to perturbations. The stability requires that nearby electric fields around $x$ should point towards $x$, implying a non-zero $\nabla\cdot E$. The differential form of Gauss's law indicates $\nabla\cdot E=\rho$ where $\rho$ is charge density. So the test particle cannot hit a vacuum point where $\rho=0$. Consequently, the particle will finally hit a point charge. Finally, we explain why the probabilities are proportional to charges.

The integral form of the Gauss's law indicates that $\int\int_{\partial \Omega} E\cdot dS=\int\int\int_{\Omega} \rho dV=0$ when the no charge is enclosed in the space $\Omega$. We define the electric flux as $\Phi=\int\int E\cdot dS$. Let us choose the pipe-like space in Figure 1(b): the `side' boundary is determined by the envelope of all electric field lines ending at $q_i$. One end (outlet) is a small ball around $q_i$, while the other end (inlet) is part of the infinite ball. The space does not have any charge inside, so the net electric flux should be zero on the whole surface, including the side, outlet and inlet. By definition the side has zero electric flux, so the amount of flux $\Phi_{in}$ that flows into the space from infinite ball should be equal to the flux $\Phi_{out}$ that flows out of the space (into the point charge $q_i$), i.e., $\Phi_{in}=\Phi_{out}$. We know $\Phi_{out}=|q_i|$ by applying Gauss's law to $q_i$. 
For the infinite ball, the inner distances among charges can be ignored, so they as a whole can be effectively viewed as a large point charge with $Q=\sum_i q_i$ placed at the origin. Denote the proportion of the pipe inlet on the whole sphere is $p_i$, which is also the probability to obtain a point on the pipe inlet when drawn from a uniform distribution on the infinite sphere. Because the effective point charge $Q$ radiates electric field isotropically on the infinite sphere, we have $\Phi_{in}=Qp_i$. To summarize, we have $Qp_i=q_i$ or $p_i=q_i/Q$.

{\bf Remark: Extending from discrete to continuous} In the discrete setting where $p(x)=\sum q_i\delta(x-x_i)/Q$ the notion of `hit' is very clear. In the continuous setting, the test particle starts from the infinite ball, moving along the electric field through space where $p(x)=0$ until hit somewhere $p(x)>0$. So the charge distribution should have compact support (otherwise $p(x)>0$ at the very beginning). 

To decide if there is a transition from $p(x)=0$ to $p(x)>0$, possible ways are: (1) adding extra auxiliary dimensions and set these dimensions to zero for data. In inference time, when these auxiliary variables are close to zero, we stop. (2) Train an extra model to inform us when to halt, for example a discriminator to decide $p(x)=0$ or $p(x)>0$. (3) After hitting, the test particle just remains there without drifting on the manifold (think of the data manifold as a sticky pad), so we can just run long enough time. This requires modifying the electric field near the pad in a clever way. This might be achieved by combining with (1). e.g, $E(x,z)=sign(z)E(x,|z|)$ ($x$ is data space, $z$ is the auxiliary variable).



\subsection{Connection to NCSN~\citep{Song2019GenerativeMB}}

\begin{align*}
    &\bm{E}(x) = \frac{1}{m}\sum_{i=1}^m \frac{x-x_i}{\parallel x-x_i\parallel_2^{n+1}}\\
    &\Longrightarrow \bm{E}(x) \propto \frac{1}{m}\sum_{i=1}^m \frac{\frac{1}{\parallel x-x_i\parallel_2^{n}}}{\sum_j \frac{1}{\parallel x-x_j\parallel_2^{n}}}  \frac{x-x_i}{\parallel x-x_i\parallel_2}\\
    &\Longrightarrow L(\theta, x) \propto \frac{1}{m}\sum_{i=1}^m \frac{1}{\parallel x-x_i\parallel_2^{n}} \parallel \bm{E}_\theta(x) - \frac{x-x_i}{\parallel x-x_i\parallel_2}\parallel_2^2\\
    &\Longrightarrow L(\theta, x) \propto \E_{x_i}\E_{x \sim \tilde{p}(x_i)}\parallel \bm{E}_\theta(x) - \frac{x-x_i}{\parallel x-x_i\parallel_2}\parallel_2^2
\end{align*}

$x_i = x + r*\Vec{v}$ where $\Vec{v}\sim \gU(\parallel \Vec{v} \parallel_2 = 1 )$,
$r \sim p(r) \propto \frac{1}{r^{n}}, r \in [a,+\infty] , p(r) = \frac{1}{r^{n}}/\int_a^\infty \frac{1}{r^{n}} dr = \frac{1}{r^{n}}/\frac{1}{n-1}a^{-(n-1)}=\frac{(n-1)a^{n-1}}{r^{n}}$. 


We can similarly deduce the optimal score function for NSCN training objective with variance $\sigma^2$:
\begin{align*}
    &L(\theta, x) \propto \frac{1}{m}\sum_{i=1}^m \exp{-\frac{\parallel x-x_i\parallel_2^2}{2\sigma^2}} \parallel s_{\theta}(x, \sigma) - \frac{x_i-x}{\sigma^2}\parallel_2^2\\
    &\Longrightarrow s^*_\theta(x, \sigma) = \sum_{i=1}^m \frac{\exp{-\frac{\parallel x-x_i\parallel_2^2}{2\sigma^2}}}{\sum_j \exp{-\frac{\parallel x-x_j\parallel_2^2}{2\sigma^2}}}  {\frac{(x_i-x)}{\sigma^2}}\\
    &\Longrightarrow s^*_\theta(x, \sigma) \propto \frac{1}{m}\sum_{i=1}^m w(i) {(x_i-x)}
\end{align*}

where $w(i) = {\exp{-\frac{\parallel x-x_i\parallel_2^2}{2\sigma^2}}}/{\sum_j \exp{-\frac{\parallel x-x_j\parallel_2^2}{2\sigma^2}}}, \sum_i w(i) = 1 $. More generally, the denoising score-matching objective is 
\begin{align*}
    \gL(\theta, \sigma) = \int p_d(x)q(x'|x)\parallel s_{\theta}(x', \sigma)- \nabla_{x'} \log q(x'|x) \parallel_2^2 dx'dx
\end{align*}
Then the optimal score has the equivalent forms:
\begin{align*}
     s_{\theta}(x', \sigma) = \frac{\int p_d(x)q(x'|x) \nabla_{x'} \log q(x'|x) dx}{\int p_d(x)q(x'|x) dx} =\frac{\int p_d(x)\nabla_{x'} q(x'|x) dx}{q(x')}={\int q(x|x')\nabla_{x'} \log q(x'|x) dx}
\end{align*}

If we plug in $q(x'|x)=\gN(x'|x, \sigma^2I)$~\citep{Song2019GenerativeMB}, the corresponding score is 
\begin{align*}
     s_{\theta}(x', \sigma) = \frac{\int p_d(x)q(x'|x) \frac{x-x'}{\sigma^2} dx}{\int p_d(x)q(x'|x) dx} =\frac{\int p_d(x)\nabla_{x'} q(x'|x) dx}{q(x')}={\int q(x|x') \frac{x-x'}{\sigma^2} dx} = \frac{1}{\sigma^2}({\int q(x|x') x dx} - x')
\end{align*}

The optimal score of finite samples $\{x_i\}_{i=1}^N$ is 
\begin{align*}
    s_{\theta}(x', \sigma) 
    &= \frac{1}{\sigma^2}({\sum_i \frac{q(x'|x_i)x_i}{\sum_j q(x'|x_j)}} - x')\\
    &= \frac{1}{\sigma^2}({\sum_i \frac{\exp{-\frac{\parallel x'-x_i\parallel_2^2}{2\sigma^2}}}{\sum_j \exp{-\frac{\parallel x'-x_j\parallel_2^2}{2\sigma^2}}} x_i} - x')\label{eq:sum_weight} \numberthis
\end{align*}

A natural question is when will dominance arise, \ie certain training samples dominate the weighted sum in \Eqref{eq:sum_weight}.

\subsection{Variational Formulation of Electricity}
The Possion's equation reads $\nabla^2\phi=-\rho$ where $\phi$ is the potential function and $\rho$ is the charge density. The energy of the electric field is defined as:

\begin{equation}
    E_f = \int dV \frac{1}{2}(\nabla\phi\cdot\nabla\phi)
\end{equation}

Consider under variation $\phi\to\phi+\delta\phi$, the variation of $E_f$ is:
\begin{equation}\label{eq:delta_Ef}
    \delta E_f = \int dV(\nabla\phi\cdot\nabla\delta\phi)=\int dV \nabla\cdot(\nabla\phi\delta\phi)-\int dV (\nabla^2\phi\delta\phi)=\int dV\rho\delta\phi
\end{equation}
where the first term vanishes due to Stokes' theorem and zero boundary condition at infinity. Define particle-field interaction energy as $E_i\equiv \int dV \rho\phi$ and the total energy as 
\begin{equation}
    E(\phi)\equiv E_f-E_i=\int dV\frac{1}{2}(\nabla\phi\cdot\nabla\phi) - \int dV\rho\phi
\end{equation}

Then Eq.~(\ref{eq:delta_Ef}) is equivalent to $\delta E=0$ (actually a minimum rather than maximum, due to physical arguments). In the MNIST setting (B=large ball, $V_B$=ball volume, $N$=number of data points, $D$:dataset),

\begin{equation}
    E(\phi)=V_{B}E_{x\in B} \frac{1}{2}||\nabla\phi(x)||_2^2 - NE_{y\sim D}\phi(y)
\end{equation}

To learn the electric potential, one can simply minimize the loss over $\phi$ (boundary condition:$\phi=0$ on the surface of the large ball).

\section{Arc length field $s(x)$}

We define $s(x)$ as the arc length function associated with each point $x$. Question: Is $\nabla s(x)$ parallel to the electric field $\nabla \phi(x)$? The answer is no. We will use proof by contradiction.

\begin{lemma}
If $\nabla s(x)$ is parallel to $\nabla \phi(x)$, then there exists a function $F:\mathbb{R}\to\mathbb{R}$, such that $\phi(x)=F(s(x))$.
\end{lemma}

\begin{proof}
$\nabla s(x)$ being parallel to $\nabla \phi(x)$ implies there exists a scalar field $a(x)$ such that $\nabla\phi(x)=a(x)\nabla s(x)$. Taking gradient gives $\nabla^T\nabla \phi(x)=\nabla^T (a(x)\nabla s(x))=a(x)\nabla^T\nabla s(x)+\nabla^T a(x)\nabla s(x)$. Note that both $\nabla^T\nabla\phi(x)$ and $\nabla^T\nabla s(x)$ are symmetric, so $\nabla^T a(s)\nabla s(x)$ should also be symmetric for all $x$. The only possibility is that there exists a $f:\mathbb{R}\to\mathbb{R}$ such that $a(s)=f(s(x))$ and hence $\nabla a(s)=\frac{df}{ds}\nabla s(x)$, $\nabla^T a(x)\nabla s(x)=\frac{df}{ds}\nabla^Ts(x)\nabla s(x)$ is symmetric. Finally, $\nabla\phi(x)=a(x)\nabla s(x)=f(s(x))\nabla s(x)=\nabla F(s(x))$ where $\frac{dF}{ds}=f$.
\end{proof}

According to the lemma, we know that for two points $x_1$ and $x_2$, as long as $s(x_1)=s(x_2)=s$, we have $\phi(x_1)=\phi(x_2)$. Since the argument is valid for all $s$, we have $\frac{d\phi}{ds}(x_1)=\frac{d\phi}{ds}(x_2)$. Recall the definition of $s(x)$, $\frac{d\phi}{ds}=E$ is the magnitude of electric field, so we have $E(x_1)=E(x_2)$. Highlighting what we have here: given $x_1\neq x_2$, as long as $\phi(x_1)=\phi(x_2)$, we have $E(x_1)=E(x_2)$, which is true only for a single point charge. A counter-example: two point charges at $x=-a$ and $x=a$. Consider $x_1=0$ and $x_2>a$ such that $\phi(x_1)=\phi(x_2)$, but we clearly have $E(x_1)=0$ and $E(x_2)>0$.

==> preliminary.tex <==
\textbf{Symbols.} We use the uppercase to denote random variable (\eg data $X$, label $Y$), the lowercase to denote the corresponding samples and the calligraphic letter to denote the sample spaces of r.v., \eg data sample space $\gX$. We focus on the setting where label space $\gY$ is discrete, \ie $\gY = \{1,\cdots,C\}$, and denote the $C-1$ dimensional probability simplex as $\Delta^{C}$. A classifier $w: \gX \to \Delta^C$ is a mapping from sample space to the simplex. It's $y$-th dimension $w(x)_y$ denotes the predicted probability of label $y$ for sample $x$. 

\textbf{Distributions.} For random variables $A,B$, we use the notation $p_A$, $p_{A|B}$, $p_{AB}$ to denote the marginal/conditional/joint distribution, \ie $p_A(a)=p(A=a)$, $p_{A|B}(a|b)=p(A=a|B=b)$,$p_{AB}(a,b)=p(A=a,B=b)$. Sometimes, for simplicity, we may ignore the subscript if there is no ambiguity, \eg $p(a|b)$ is an abbreviation for $p_{A|B}(a|b)$.


We begin by defining the notion of an orthogonal random variable. We consider continuous $X,Z_1,Z_2$ and assume their supports are manifolds diffeomorphic with the Euclidean space. The probability density functions~(PDF) are in $\gC^1$. 
% \hhh{What are all sample spaces?} 
Given a joint distribution $p_{XY}$, we define the orthogonal random variable as follows:
\begin{definition}[Orthogonal random variables] \label{def:orth} We say $Z_1$ and $Z_2$ are orthogonal random variables w.r.t $p_{XY}$ if they satisfy the following properties:
\begin{enumerate}[(i)]
    \item There exists a diffeomorphism $f:\gZ_1 \times 
    \gZ_2 \to \gX$ such that $f(Z_1,Z_2)=X$.
    \item $Z_1$ and $Z_2$ are statistically independent given $Y$, \ie $Z_1 \indep Z_2 | Y$.
\end{enumerate}
\end{definition}




The orthogonality relation is symmetric by definition. %We say $Z_1,Z_2$ are \emph{mutually orthogonal} if they satisfy the properties in definition \ref{def:orth}. 
Note that the orthogonal pair perfectly reconstructs the observations via diffeomorphism $f$; as random variables they are also sampled independently from class conditional distributions $p(Z_1|Y)$ and $p(Z_2|Y)$. For example, we can regard foreground objects and background scenes in natural images as being mutually orthogonal random variables. 

\paragraph{Remark.} The definition of orthogonality can be similarly developed for the discrete variables and discrete-continuous mixtures. For discrete variables, for example, we can replace the requirement of diffeomorphism with bijection. 
% TJ: this needs to be clarified or delete (as I did here)
%For discrete-continuous mixtures, we would need to require that require $Z_1$ to has one-to-one correspondence with the discrete component, and $Z_2$ and the continuous component are diffeomorphic, or vice versa.

Since the diffeomorphism $f$ is invertible, we can use $z_1:\gX\to \gZ_1$ and $z_2:\gX \to \gZ_2$ to denote the two parts of the inverse mapping so that $Z_1=z_1(X)$ and $Z_2=z_2(X)$. Note that, for a given joint distribution $p_{XY}$, the decomposition into  orthogonal random variables is not unique. There are multiple pairs of random variables that represent valid mutually orthogonal latents of the data. 
We can further justify our definition of orthogonality from an information theoretic perspective by showing that the choice of $z_2$ attains the maximum of the following constrained optimization problem. 
% Given a random variable $z_1(X)$, we want to find another random variable that is predictive of $Y$ meanwhile represents aspects other than $z_1(X)$. Rigorously, our goal is to find a function $z =\argmax_z I(z(X),Y|z_1(X)), \textrm{s.t. } I(z(X); z_1(X)|Y)=0$. We show that the orthogonal random variable $z_2(X)$ is the optimal function.

\begin{restatable}{proposition}{info}
\label{prop:info}
Suppose the orthogonal r.v. of $z_1(X)$ w.r.t $p_{XY}$ exists and is denoted as $z_2(X)$. Then $z(X) = z_2(X)$ is a maximizer of $I(z(X),Y|z_1(X))$ subject to $I(z(X); z_1(X)|Y)=0$. 
\end{restatable}

\newcommand{\finvone}{f^{-1}_1}
\newcommand{\finvtwo}{f^{-1}_2}
% We assume the data have the following generating process. First, label $Y$ is sampled from the label distribution $p(Y)$. 
% Since the two latent orthogonal random variables $Z_1, Z_2$ are independently generated from the conditional distributions $p(Z_1|Y)$ and $p(Z_2|Y)$, and the observation $X$ is generated via a diffeomorphism mapping $f$ from $Z_1, Z_2$, \ie $X=f(Z_1,Z_2)$. 

% Since the diffeomorphism $f$ is invertible, we use $f^{-1}_1$ and $f^{-1}_2$ to denote the two parts of the inverse mapping that correspond to the two r.v., \ie $Z_1=f^{-1}_1(X)$ and $Z_2=f^{-1}_2(X)$. We call $Z_1,Z_2$ as mutually orthogonal latent for the data $X,Y$. Note that, for a given data distribution, the generating process the not unique. There might be multiple mutually orthogonal random variables can be served as the latent of the data.


% Since $f$ is diffeomorphism, it is in principal possible to recover the latents from the observations, \ie there exists an inverse mapping, $f^{-1}(x)=(z_1,z_2)$. By the change of volume, the pdf for $x$ in the $i$-th class is $p_i(x) = p_i(z_1,z_2)k(z_1,z_2)$ where $k(z_1,z_2)$ is the ratio of volume determined by $f$.

We defer the proof to Appendix~\ref{app:info-proof}. Proposition~\ref{prop:info} shows that the orthogonal random variable maximizes the additional information about the label we can obtain from $X$ while remaining conditionally independent of the principal random variable. This ensures complementary in predicting the label. 





% We denote the label-conditioned data/latent distributions as $p_y(x)=p(X=x|Y=y)$, $p_{y,1}(z_1)=p(Z_1=z_1|Y=y)$ and $p_{y,2}(z_2)=p(Z_2=z_2|Y=y)$ for clarity.  

% The classifier $w_1$ is defined as the Bayesian optimal classifier using only $Z_1$ for prediction, \ie $w_1: \gX \to \Delta^{C}$ and $w_1(x)_y = p(Y=y|z_1(x))$. Similarly, we define orthogonal classifier $w_2$ as the Bayesian optimal classifier only using $Z_2$, \ie $w_2(x)_y = p(Y=y|z_2(x))$ and full classifier $w_x$ which uses full information of $x$,  \ie $w_x(x)_y = p(Y=y|x)$.

==> related_works.tex <==
% \red{disentanglement (define useful disentanglement), fairness(calculation)}

\paragraph{Disentangled representation learning} Similar to orthogonal random variables, disentangled representation learning associates a definition of independence of dimensions in the representation. \citet{Higgins2018TowardsAD} defines the disentangled representations based on the equivalence and independence of group transformations, \citet{Kim2018DisentanglingBF} relates disentanglement to distribution factorization and \citet{Shu2018ADA} characterizes disentanglement via generator consistency and restrictiveness. There are two key differences. First, most disentanglement definitions do not take the diffeomorphism and the labels into account. In contrast, our definition requires diffeomorphism and label-conditioned independence. Further, disentanglement learning does not learn discriminative models on different latents as ours. Several works aim to learn the disentangled representations~\citep{Chen2016InfoGANIR,Higgins2017betaVAELB,Chen2018IsolatingSO}. However, \cite{Locatello2019ChallengingCA} shows that unsupervised learning of disentangled representation is impossible without inductive bias.
\paragraph{Model debiasing}
A line of works focuses on prevent model replying on the dataset biases. \citet{Bahng2020LearningDR} learns the debiased representation by imposing HSIC penalty with designed biased representation, and \citet{Nam2020LearningFF} trains an unbiased model by up-weighting the high loss samples in the biased model. \citet{Li2021ShapeTextureDN} de-bias training data through data augmentation. However, these works lack theoretical definition for the debiased model in general cases and often require explicit dataset biases. 
\paragraph{Density ratio estimation using classifier} Using binary classifier for estimating the density ratio~\citep{Sugiyama2012DensityRE} enjoys widespread attention in machine learning. The density ratio estimated by classifier has been applied to Monte Carlo inference~\citep{Grover2019BiasCO,Azadi2019DiscriminatorRS}, class imbalance~\citep{Byrd2019WhatIT} and domain adaptation~\citep{Azizzadenesheli2019RegularizedLF}.

